ConDor: Self-Supervised Canonicalization of 3D Pose for Partial Shapes

Progress in 3D object understanding has relied on manually canonicalized shape datasets that contain instances with consistent position and orientation (3D pose). This has made it hard to generalize these methods to in-the-wild shapes, eg., from internet model collections or depth sensors. ConDor is a self-supervised method that learns to Canonicalize the 3D orientation and position for full and partial 3D point clouds. We build on top of Tensor Field Networks (TFNs), a class of permutation- and rotation-equivariant, and translation-invariant 3D networks. During inference, our method takes an unseen full or partial 3D point cloud at an arbitrary pose and outputs an equivariant canonical pose. During training, this network uses self-supervision losses to learn the canonical pose from an un-canonicalized collection of full and partial 3D point clouds. ConDor can also learn to consistently co-segment object parts without any supervision. Extensive quantitative results on four new metrics show that our approach outperforms existing methods while enabling new applications such as operation on depth images and annotation transfer.

==> content/Arxiv/affiliation.tex <==
\footnotetext[1]{Robotics Research Center, IIIT Hyderabad, India}
\footnotetext[2]{Stanford University, USA}
\footnotetext[3]{KAIST, South Korea}
\footnotetext[4]{Brown University, USA}

==> content/arch.tex <==
\begin{figure}[H]
\centering
  \includegraphics[width=0.5\textwidth, trim={5cm 1cm 5cm 1cm},clip]{images/Partial canonical capsules.jpg}
  \caption{Tensor Field Capsules pictorial representation}
  \label{fig:partial_canonical_tfn}
\end{figure}

==> content/loss.tex <==
\begin{itemize}
    \item L2 Loss ($Y(v(X))$ must be equal to $v(X)$ up to rotation):
    \[
    \frac{2}{N}\sum_i \Vert v(X)_{i,:} - U(v(X))V(v(X))Y_{i,:}(v(X)) \Vert_2^2
    \]
    % \item L2 restriction loss: ($Y(v(X))$ must be equal to $Y^{\mathrm{full}}(v(X))$):
    % \[
    % \frac{2}{N}\sum_i \Vert Y^{\mathrm{full}}_{i,:}(v(X)) - Y_{i,:}(v(X)) \Vert_2^2
    % \]
    % \item Capsules restriction loss: ($S(v(X))$ must be equal to $S^{\mathrm{full}}(v(X))$):
    % \[
    % \frac{2}{N}\sum_i \mathrm{crossentropy}(S^{\mathrm{full}}_{i,:}(v(X)), S_{i,:}(v(X))) 
    % \]
    \item Orthonormality loss ($E(v(X))$ should be an orthonormal basis):
    \[
    \Vert U(v(X))V(v(X)) - E(v(X))\Vert_2
    \]
    \item \textbf{Position loss for centroids}: Centroids $\theta(v(X), v(S^{full}_{i, :}))$ should be the same as $\theta(v(X), S_{i, :})$. (Even though the input ($v(X)$) is the same, the capsule weights $S$ are computed on full shape and sliced ($S^{full}_{i, :}$) vs. computed on partial shape ($S^{full}_{i, :}$):
    \begin{equation}
        \left|\left|\theta(v(X), v(S^{full}_{i, :})) - \theta(v(X), S_{i, :})\right|\right|_1
    \end{equation}
    \item \textbf{Directional loss for centroids}: Inter-centroid directions obtained by restriction of the full shape prediction and the partial shape prediction should be equivalent. $dir(\theta(X, S))$ computes the vector directions between every $^{n}C_2$ centroid pairs. 
    \begin{equation}
        1 - \mathrm{cosine\_similarity}(dir(\theta(v(X), v(S^{full}_{i, :}))), dir(\theta(v(X), S_{i, :})))
    \end{equation}
    
    \item \textbf{Capsule categorical loss}: This loss tries to ensure that for every point in the point cloud, its maximum mass lies within a particular capsule. Let $S^{b}_{i, :}(S^{full})$ represent the capsule predictions for a point cloud with the capsule that is activated the most be labelled as $1$ and the remaining capsule positions labelled as $0$. We obtain the maximum activated capsule using the network's prediction itself.
    \begin{equation}
        \mathrm{CategoricalCrossEntropy}(S^{b}_{i, :}(S^{full}_{i, :}), S^{full}_{i, :})    
    \end{equation}
    
    % \item \textbf{Eigen reconstruction loss}: We have seen some failure cases where the object shrinks or stretches along one of the dimensions. We employ SVD and ensure that the Eigenvalues across the two shapes are the same to avoid the scaling caused in TFN capsules.
    % \[
    % D, U, V = SVD(X)
    % \]
    % \[
    % D_{p}, U_{p}, V_{p} = SVD(E(X)Y(X))
    % \]
    % \begin{equation}
    %     \left| \left| D - D_{p}\right|\right|_2
    % \end{equation}
    
    % \item \textbf{Pose loss}: The pose obtained for the partial pointcloud should be the same as the pose obtained for the complete pointcloud.
    % \begin{equation}
    %     \left| \left| E(X) - E(v(X))\right| \right|_2 + \sum_i 1 - \mathrm{cosine\_similarity(E(X)_{:, i}, E(v(X))_{:, i})}
    % \end{equation}
\end{itemize}

==> content/text/tables/ablation_loss_functions.tex <==
% \begingroup
\setlength{\intextsep}{0pt}%
\setlength{\columnsep}{5pt}%
\begin{wraptable}{r}{0.6\columnwidth}
\vspace{0.05in}
\caption{Ablating the separation and restriction losses.
% loss functions: ``w/o sep'' ($\mathcal{L}_{sep}$) and ``w/o rest'' denote training without separation and without restriction loss. respectively.
\label{table:loss_ablation}}
\vspace{-0.1in}
\centering
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
% \textbf{Category}  $\rightarrow$
& \multicolumn{3}{c}{\textbf{Avg. (plane, table, chair)}}\\ 
\midrule
% \textbf{Metric} $\downarrow$        
& \textbf{Ours} & \textbf{w/o $\mathcal{L}_{sep}$} & \textbf{w/o $\mathcal{L}_{rest}$} \\ \midrule
\multicolumn{1}{l|}{GC (full) {\color{blue} $\downarrow$}}     & 0.0511         & 0.0464        & 0.0521  \\ %\hline

\multicolumn{1}{l|}{IC (full) {\color{blue} $\downarrow$}}      &0.0247         &0.0341        &0.0275 \\ %\hline

\multicolumn{1}{l|}{CC (full) {\color{blue} $\downarrow$}}    &0.1085         &0.1119        &0.1087  \\ %\hline
\midrule
\multicolumn{1}{l|}{GC (partial) {\color{blue} $\downarrow$}}  &0.0601                  &0.0531        &0.0622 \\ %\hline
\multicolumn{1}{l|}{IC (partial) {\color{blue} $\downarrow$}}   &0.0542         &0.0551        &0.0708  \\ %\hline
\multicolumn{1}{l|}{CC (partial) {\color{blue} $\downarrow$}} &0.1187         &0.1191        &0.1247 \\ 
\midrule
\multicolumn{1}{l|}{Average {\color{blue} $\downarrow$}} &\textbf{0.0696}         &0.0700        &0.0743 \\ 
\bottomrule
\end{tabular}
}
\vspace{-0.05in}
\end{wraptable}
% \endgroup

==> content/text/tables/all_ablations.tex <==
\begin{table}[!h]
\centering
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
% \textbf{Category}  $\rightarrow$
& \multicolumn{3}{c}{\textbf{Avg. (Plane, Table, Chair)}}\\ 
\midrule
% \textbf{Metric} $\downarrow$        
& \textbf{Ours} & \textbf{w/o $\mathcal{L}_{sep}$} & \textbf{w/o $\mathcal{L}_{rest}$} \\ \midrule
\multicolumn{1}{l|}{GC (full)}     & 0.0511         & 0.0464        & 0.0521  \\ %\hline

\multicolumn{1}{l|}{IC (full)}      &0.0247         &0.0341        &0.0275 \\ %\hline

\multicolumn{1}{l|}{CC (full)}    &0.1085         &0.1119        &0.1087  \\ %\hline
\midrule
\multicolumn{1}{l|}{GC (partial)}  &0.0601                  &0.0531        &0.0622 \\ %\hline
\multicolumn{1}{l|}{IC (partial)}   &0.0542         &0.0551        &0.0708  \\ %\hline
\multicolumn{1}{l|}{CC (partial)} &0.1187         &0.1191        &0.1247 \\ 
\midrule
\multicolumn{1}{l|}{Average} &\textbf{0.0696}         &0.0700        &0.0743 \\ 
\bottomrule
\end{tabular}
}
\caption{Ablating the benefit of the separation and restriction losses.
% loss functions: ``w/o sep'' ($\mathcal{L}_{sep}$) and ``w/o rest'' denote training without separation and without restriction loss. respectively.
\label{table:loss_ablation}}
\end{table}


% \begin{table}[h]
% \centering
% \scalebox{0.7}{
% \begin{tabular}{c|cccc}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Test partiality}}}                          & \multicolumn{4}{c}{\textbf{Degree of partiality during training}}                                  \\ \cline{2-5} 
% \multicolumn{1}{c|}{}                                                          & \multicolumn{1}{c}{1/4} & \multicolumn{1}{c}{1/2} & \multicolumn{1}{c}{3/4} & {[}1/4, 3/4{]}  \\ \midrule
% \multicolumn{5}{l}{\textbf{Instance-Level Consistency (IC)}{\color{blue} $\downarrow$}} \\
% \midrule
% % \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{IC (partial)}}}   &
% \multicolumn{1}{l|}{1/4}            & 0.0728                   & \textbf{0.0719}          & 0.1542                   & 0.0797          \\ %\cline{2-6} 
% % \multicolumn{1}{c|}{}                                         & 
% \multicolumn{1}{l|}{1/2}            & 0.0452                   & \textbf{0.0349}          & 0.0526                   & 0.0380          \\ %\cline{2-6} 
% % \multicolumn{1}{c|}{}                                         & 
% \multicolumn{1}{l|}{3/4}            & 0.0456                   & 0.0333                   & \textbf{0.0221}          & 0.0334          \\ %\cline{2-6} 
% % \multicolumn{1}{c|}{}                                         & 
% \multicolumn{1}{l|}{{[}1/4, 3/4{]}} & \textbf{0.0719}          & 0.0792                   & 0.1049                   & 0.0804          \\ \midrule
% \multicolumn{5}{l}{\textbf{Category-Level Consistency (CC)}{\color{blue} $\downarrow$}} \\
% \midrule
% % \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{CC (partial)}}} & 
% \multicolumn{1}{l|}{1/4}            & 0.0914                   & \textbf{0.0895}          & 0.1702                   & 0.0966          \\ %\cline{2-6} 
% % \multicolumn{1}{c|}{}                                         & 
% \multicolumn{1}{l|}{1/2}            & 0.0652                   & 0.0632                   & 0.0731                   & \textbf{0.0617} \\ %\cline{2-6} 
% % \multicolumn{1}{c|}{}                                         & 
% \multicolumn{1}{l|}{3/4}            & 0.0657                   & 0.0608                   & \textbf{0.0582}          & 0.0606          \\ %\cline{2-6} 
% % \multicolumn{1}{c|}{}                                         & 
% \multicolumn{1}{l|}{{[}1/4, 3/4{]}} & \textbf{0.0895}          & 0.0985                   & 0.1216                   & 0.0982          \\ \midrule
% % \hline
% \multicolumn{1}{l|}{\textbf{Average}}                                          & 0.0594                   & \textbf{0.0580}          & 0.0886                   & 0.0610          \\ \midrule
% \end{tabular}
% }
% \caption{\textbf{Degree of partiality} - Partiality introduced during training (vertical) is evaluated on the canonicalization metrics with different fraction of partiality (horizontal). Our model trained with partiality $1/2$ performs better on average over all the canonicalization metrics.\label{table:deg_partiality}}
% \end{table}
